FastPoints: A State-of-the-Art Point Cloud Renderer for Unity

In this paper, we introduce FastPoints, a state-of-the-art point cloud renderer for the Unity game development platform. Our program supports standard unprocessed point cloud formats with non-programmatic, drag-and-drop support, and creates an out-of-core data structure for large clouds without requiring an explicit preprocessing step; instead, the software renders a decimated point cloud immediately and constructs a shallow octree online, during which time the Unity editor remains fully interactive.

==> alt-sections/future-work.tex <==
\section{Future Work}

One advantage of the choice of Unity as a development platform is that it offers a robust suite of tools for extending FastPoints and improving the plugin in a variety of ways.

For the core rendering pipeline, one planned feature is the inclusion of progressive rendering as described by Schütz et. al. \cite{schutz2020progressive} This would allow significantly more points to be sent to the GPU without as many visible artifacts as exist with the current chunk-by-chunk loading of points. An initial large sparse cloud could be loaded to the GPU progressively over the course of multiple frames, and then using the reproject-fill-prepare loop described, more points could be loaded only as needed while the majority remain in GPU memory between frames.

Other planned features include adaptive point sizing, specifically for the initial decimated cloud, as well as point blending and eye dome lighting.

Additionally, while the primary focus of this tool thus far has been user experience and high-level design, we hope to extend the tool with a more performant low-level interface to enhance the speed and flexibility of the project even further. Specifically, the tool currently interfaces with LAStools on the native side to handle cloud decimation and PLY conversion. While this performs extremely well for decimating and processing LAS and LAZ files, results with PLY files could be improved. For instance, the PLY-to-LAS conversion step could be avoided completely with an implementation of the Potree Converter that supports PLY files. Additionally, LAStools' PLY reader is designed to parse LAS attributes such as bounds that are unnecessary for the decimation step of our program; a custom implementation of a PLY reader could significantly reduce the time needed for subsampling PLY files.

More research could also be done in the sampling method for the initial decimated cloud. While uniform sampling was chosen for this application to maximize subsampling speed, one could imagine point clouds that are ordered such that uniform sampling results in unevenly distributed points in the decimated cloud. While none of the clouds we tested had this issue, if this becomes an issue in the future, it could be handled by a spatially-constrained random sampler.

==> alt-sections/implementation.tex <==
\section{Implementation}

Our tool utilizes a C\# plugin for interfacing with Unity as well as a native C++ plugin for most hefty IO operations and interaction with C++ conversion tools.

\subsection{File Importing}

For file importing, we utilize Unity's asset pipeline to support drag-and-drop importing of unordered point cloud PLY, LAS, or LAZ files. When a file is added, the plugin initializes a handle object for IO operations that can be passed to the C++ side of the plugin and starts conversion and octree construction operations.

\subsection{Immediate Low-Resolution Rendering}

Once the handle asset has been initialized, the program begins point cloud decimation. This requires iterating over the entire point cloud to sample uniformly and thus has time requirements that are roughly linear with respect to point cloud size. To minimize the amount of time this step takes, we spawn multiple threads to subsample different chunks of the point cloud simultaneously and leverage the speed of modern SSDs. Since point cloud conversion and decimation scales with cloud size as well, the result is an additional subsampling step that is consistently far quicker than the full octree construction, usually finishing in a matter of seconds even for clouds with hundreds of millions of points.

One consideration with this step is the difference in performance between point cloud formats. While both PLY and LAS files can be iterated over and parsed quickly, LAZ files require a point-wise decoding to parse position and color attributes. This causes a significant time increase in decimation, but since this decoding is also necessary for octree construction, the total time for decimation remains a small proportion of the overall preprocessing time.

\subsection{File Conversion}

While the Potree Converter supports LAS and LAZ files out-of-the-box, it lacks support for PLY files. To address this, we include an additional conversion step for PLY files, using LAStools' las2las program to create temporary las files that can be used with the Potree Converter then cleaned up after the octree is constructed. This means processing times are longer for PLY files than LAS or LAZ files, but due to our program architecture, the decimated cloud is fully interactive for the duration of this additional conversion phase as well.

\subsection{Octree Construction}

Once the initial decimated cloud is done, an octree is constructed by the Potree Converter  described by Schütz et. al. \cite{schutz2020fast} First, the point cloud is sorted into a number of out-of-core chunks; then, the chunks are read back and converted into local octrees in parallel; finally, the local octrees are stitched together into a global octree that is written to a single file.

Our program runs the potree converter with larger per-node point counts than the default settings, avoiding recursive calls normally performed to break up large nodes and reducing the number of distinct IO calls needed to transfer the points of each node to disk.

Once construction is complete, the resulting files are linked to the created Unity asset, allowing entire asset to be transferred between Unity projects seamlessly without losing access to the original point cloud.

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.5\columnwidth]{octree.drawio.png}
    \caption{Octree construction pipeline, as described by Schütz et. al. The imported file is first sorted into a number of out-of-core chunk files, each representing a node in the global tree. The chunks are then indexed in parallel, creating local octrees, whose points are written to an additional file. Finally, the octrees are stitched together into a global tree, and the entire structure is written to an additional file.}
\end{figure*}

\subsection{Octree Rendering}

Once the entire octree is written to disk, the original decimated cloud is cleared from memory and the octree skeleton is used to render points from the generated structure using the current camera position. 

To avoid slowing the main thread during octree traversal, we create a separate traversal thread that walks the tree and checks each node's visibility. If a node should be rendered, the traverser checks if its points are loaded from disk. If they are, the node is added to a queue of nodes to be rendered; if not, the node is marked and its points are asynchronously loaded into a Unity ComputeBuffer object allocated directly on the GPU. Conversely, if a node has points loaded but is not visible in the frame, its points are discarded to free GPU memory. Once the tree is fully traversed, the newly populated node queue is sent to the main thread.

The main thread executes its work in the Unity per-frame Update and OnRenderObject methods. Each frame, the main thread sends frustum and positional camera information to the traverser thread, fetches the most recently sent node queue, and iterates through the queue. Each node is passed to a compute shader that populates a single texture with depth and color information, processing points far more quickly than a standard rasterization pipeline using the early depth testing and the busy-wait loop technique described in Günther et. al. 2013. \cite{gunther2013gpgpu} Once all nodes have been rendered to this texture, color and depth textures are fetched from Unity's currently rendering camera and a final rendered texture is created from the per-pixel minimum depths of the main camera texture and the render point cloud texture.

One challenge we faced with this architecture was that Unity's API is single-threaded, meaning any calls interacting with Unity objects, including cameras and Compute Buffers, must be done on the main thread, which blocks the editor if an operation takes too much time. We implemented a variant of a multi-threaded queue to allow small function calls to be encapsulated in C\# Action objects and queued for execution on the main thread, which processes a fixed number of Actions each frame to avoid blocking.

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.4\columnwidth]{render.drawio.png}
    \caption{Overview of our CPU-side octree rendering algorithm. A spawned thread receives camera position and frustum data from the main thread, then traverses the octree, loading points into all nodes that are in-frame. The main thread, meanwhile, reads loaded points from the octree each frame and writes them to a GPU buffer.}
\end{figure*}

==> alt-sections/introduction.tex <==
\section{Introduction}

Over the past decade, as laser scanners have become more accessible and graphics cards have become more powerful, the point cloud data format has seen a significant increase in popularity. With this new popularity has come a host of new aspiring users of point clouds, including many who hope to integrate point clouds with other types of visualizations, whether those are static meshes, sprites, or voxels. While the most technically advanced and performant point cloud renderers available today are dedicated point cloud tools without support for other popular graphics formats, some developers have focused on integrating point cloud rendering with existing graphical development platforms to support a wider array of rendering functionality in conjunction with point cloud visualization.

One of the most pervasive challenges in point cloud rendering is the visualization of clouds that are too large to be stored in main or GPU memory. While small point clouds that can be stored fully in RAM pose few challenges for a rendering application, large point clouds that can only be loaded partially into memory at any one time create significant complications. A renderer must select subsets of the point cloud on a frame-by-frame basis, loading only the points that should be rendered immediately into memory. One way to accomplish this is to create a level-of-detail out-of-core data structure for these clouds, such as an octree or a kd-tree, and store sub-clouds in the nodes of the tree itself to be loaded at runtime. Many state-of-the-art tools leverage these LOD structures, but these require explicit preprocessing operations that often aren't integrated with rendering tools, forcing users to wait long periods of time before they're able to view their point clouds and possibly install external tools to create the data structure.

Additionally, a number of tools support LOD structures with sophisticated CPU-side algorithms, but don't take advantage of recent GPU-side improvements in point cloud rendering technology. This forces generated data structures to have high granularity and thus require more preprocessing time to ensure each draw call doesn't overexert the GPU.

In this thesis, a new tool is presented to integrate with the Unity3D platform and allow immediate visualization of a decimated point cloud and online data structure generation with tighter integration than any alternative available for Unity. This tool, FastPoints, offers a number of benefits to user experience compared to other large point cloud viewers and Unity point cloud renderers:


\begin{itemize}
    \item Fully non-programmatic interface
    \item Integrable With Standard Mesh Rendering Pipelines
    \item Interactive During Preprocessing
    \item Support for Popular Point Cloud Formats
\end{itemize}

\begin{table*}[b]
    \centering
    \begin{tabular}{|c||c|c|c|c|c|}
        \hline
            Method & 
            \begin{tabular}{@{}c@{}}Large point \\ cloud support\end{tabular} & \begin{tabular}{@{}c@{}} Unity \\ Integration\end{tabular} & \begin{tabular}{@{}c@{}}Interactive during \\ preprocessing\end{tabular} &
            \begin{tabular}{@{}c@{}}Non-programmatic \\ interface\end{tabular} &
            \begin{tabular}{@{}c@{}}Support for \\ LAS, LAZ, \\ and PLY files\end{tabular}\\
        \hline
        pcx & \XSolid & \Checkmark & N/A & \Checkmark & \XSolid \\
        \hline
        Potree & \Checkmark & \XSolid & \XSolid & \XSolid & \XSolid \\
        \hline
        BA\_PointCloud & \Checkmark & \Checkmark & \XSolid & \XSolid& \XSolid \\
        \hline
        FastPoints & \Checkmark & \Checkmark & \Checkmark & \Checkmark& \Checkmark \\
        \hline
    \end{tabular}
    \caption{Feature Comparison of Existing Point Cloud Renderers}
    \label{tab:my_label}
\end{table*}

==> alt-sections/program-structure.tex <==

\section{Program Structure}
FastPoints, the method presented, introduces a novel program structure that incorporates a number of recent developments in point cloud rendering research to avoid some of the limitations of existing point cloud rendering solutions. Specifically, we prioritize seamless user experience, immediate interactivity, support for popular point cloud formats, and tight integration with the Unity environment.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{pointcloud2.png}
    \caption{Full detail on the statue and surrounding furnishings after octree construction}
\end{figure}

To support seamless user experience, we integrate our plugin with Unity's built-in asset pipeline to allow for drag-and-drop importing of unstructured point cloud formats such as PLY, LAS, or LAZ files. Once a cloud has been imported, we provide immediate interactivity by uniformly downsampling the cloud and rendering the result. This gives users a rough approximation of their implemented cloud while further preprocessing is performed.

After the initial downsampling step, we generate an out-of-core octree using the Potree Converter 2.0 described by Schütz et. al. in 2020. \cite{schutz2020fast} During this time, the Unity environment and the initial downsampled cloud remain fully interactive, allowing users to position their point clouds in larger scenes or continue to work on other aspects of their project. To reduce preprocessing time, we generate an octree that is shallower than many other implementations, sometimes containing hundreds of thousands of points per node. This decision is possible due to the improved rendering methods implemented for the plugin which can support larger point counts loaded per frame.

Once the octree is fully generated, we discard the decimated point cloud and traverse the octree, dynamically loading points based on the camera position each frame. Due to the shallowness of the generated tree, the number of points loaded per traversal is large on average, but small camera adjustments often keep the same nodes in-frame and do not require reloading points at all. To accommodate this higher per-frame point count in the case where large camera movements lead to significant reloading between frames, FastPoints leverages the GPGPU technique described by Günther et. al. in 2013 \cite{gunther2013gpgpu}.

\begin{figure}[t]
    \centering
    \includegraphics[width=.9\columnwidth]{algorithm.drawio.png}
    \caption{Our overall program structure. Point clouds are imported, then, if no octree has been constructed previously, the cloud is decimated for immediate rendering on the main thread and a new thread spawns to construct the octree. Once the tree is done, the decimated cloud is discarded and the octree is rendered in its place.}
\end{figure}
